Towards Theoretical Understandings of Robust Markov Decision Processes: Sample Complexity and Asymptotics

In this paper, we study the non-asymptotic and asymptotic performances of the optimal robust policy and value function of robust Markov Decision Processes(MDPs), where the optimal robust policy and value function are solved only from a generative model. While prior work focusing on non-asymptotic performances of robust MDPs is restricted in the setting of the KL uncertainty set and $(s,a)$-rectangular assumption, we improve their results and also consider other uncertainty sets, including $L_1$ and $\chi^2$ balls. Our results show that when we assume $(s,a)$-rectangular on uncertainty sets, the sample complexity is about $\widetilde{O}\left(\frac{|\mathcal{S}|^2|\mathcal{A}|}{\varepsilon^2\rho^2(1-\gamma)^4}\right)$. In addition, we extend our results from $(s,a)$-rectangular assumption to $s$-rectangular assumption. In this scenario, the sample complexity varies with the choice of uncertainty sets and is generally larger than the case under $(s,a)$-rectangular assumption. Moreover, we also show that the optimal robust value function is asymptotic normal with a typical rate $\sqrt{n}$ under $(s,a)$ and $s$-rectangular assumptions from both theoretical and empirical perspectives.

==> tex/acknow.tex <==
The authors thank Xiang Li and Dachao Lin for a discussion related to DRO and some inequalities.

==> tex/apdix/changes.tex <==
Before the point-by-point responses to reviewers' comments, we would like to list the major changes we have made in this revision.

% \section*{\textbf{A. A footnote about a recent paper \cite{panaganti2021sample} with similar results on Page 4}}

% We appreciate that Reviewer 1 reminds us a recent paper \cite{panaganti2021sample} appeared online during the reviewing process of our manuscript. Indeed, \citet{panaganti2021sample} only prove the finite-sample results under $(s,a)$-rectangular assumption, which have a worse dependence on $(1-\gamma)^{-1}$ than our results, while we consider a more complicated setting and also give asymptotic results. In the revision, we add a footnote about this paper on Page 4. 

\section*{\textbf{A. Description of $(s,a)$-rectangular and $s$-rectangular assumptions}}

Both reviewers find that the Assumption~\ref{asmp: sa-rect} and \ref{asmp: s-rect} could be confusing. In the revised version, we follow the prior works' notations to give a more precise description of $(s,a)$-rectangular and $s$-rectangular assumptions on Page 5-6.

\section*{\textbf{B. ``Connection with non-robust MDPs'' in Section 2, Page 6-7}}

In the revised version, we discuss how the size of the uncertainty set $\rho$ controls the distance between robust value function $V_r^\pi$ and non-robust value function $V^\pi$. With a small $\rho$, Theorem~\ref{thm: non-robust-difference} implies the robust value function $V_r^\pi$ can be really close to the non-robust value function $V^\pi_{P^*}$, where $\|V_r^\pi - V^\pi_{P^*}\|_\infty\le O(h(\rho))$, where $h(\cdot)$ is a continuous monotonically increasing function and $h(0)=0$. This part enables us to discuss the finite-sample bounds of the robust value function when $\rho\to 0$ in Section~\ref{subsec: discussrho}.

\section*{\textbf{C. Proof sketch of finite-sample results and asymtotic results in Section~\ref{sec: gen} and Section~\ref{sec: asymp}}}

In the revised version, we also add proof sketches of finite-sample results and asymptotic results at the beginning of Section~\ref{sec: gen} and Section~\ref{sec: asymp}, respectively.
We hope this could provide more intuition and make it easier for the readers to understand our results.

\section*{\textbf{D. Concatenated theoretical results in Section~\ref{sec: gen} and Section~\ref{sec: asymp}}}

To make our manuscript more readable, in the revised version, we concatenate our finite-sample results as well as asymptotic results under different choices of ambiguity sets ($L_1$, $\chi^2$, and KL).
The concatenated results can be found in Theorem~\ref{thm: finite-sa} (finite-sample results under $(s,a)$-rectangular assumption), Theorem~\ref{thm: finite-s} (finite-sample results under $s$-rectangular assumption), Theorem~\ref{thm: normal-sa} (asymptotic results under $(s,a)$-rectangular assumption), and Theorem~\ref{thm: normal-s} (asymptotic results under $s$-rectangular assumption).

\section*{\textbf{E. Discussion on finite-sample results in Section~\ref{subsec: discussrho}}}

In the revised version, we add a new subsection (subsection~\ref{subsec: discussrho}) discussing our finite-sample results, especially in the case of $\rho\to 0$. Specifically, the sample complexity bounds in Theorem~\ref{thm: finite-sa} and Theorem~\ref{thm: finite-s} would be infinitely large when $\rho$ goes zero. In section~\ref{subsec: discussrho}, we give a simple distributionally robust optimization problem to illustrate why this phenomenon occurs. We also show that such issues can be alleviated by combining Theorem~\ref{thm: non-robust-difference} and sample complexity bounds in non-robust MDPs.

\section*{\textbf{F. Discussion on the gap between the upper and lower bound in Section~\ref{sec: lb}}}

In the revised version, we add a new paragraph (Section~\ref{sec: lb}) to discuss the possible reason why a gap exists between the upper bound and lower bound in Section~\ref{sec: gen}.

\section*{\textbf{G. Discussion on asymptotic results in Section~\ref{subsec: discussasympvar}}}

In the revised version, we add a new subsection (subsection~\ref{subsec: discussasympvar}) interpreting the asymptotic variance of the estimated value functions of robust MDPs. Specifically, we compare our asymptotic variances with their counterparts in non-robust MDPs and propose methods to construct confidence intervals from our asymptotic results. 

\section*{\textbf{F. Order of references}}

In the revised version, we rearrange the order of references in the main text.

==> tex/apdix/relwork.tex <==
\paragraph{Offline RL.} Offline RL mainly is divided into two parts: Off-Policy Evaluation (OPE) and Off-Policy Learning (OPL). Both of these two problems assume the agent is unable to interact with the environment but only access to a given explorable dataset. In terms of OPE, there are mainly three different methods: Direct Method (DM), Importance Sampling (IS), and Doubly Robust (DR). For DM, the approach is directly estimating the value function from the dataset and evaluating value function under a given target policy \citep{mannor2004bias, jong2007model, grunewalder2012modelling, bertsekas1995neuro, dann2014policy, duan2020minimax}. 
The second approach is IS, or its variant self-normalized IS, where the density ratio of evaluation and target policies is estimated from dataset \citep{hirano2003efficient, li2015toward, liu2018breaking, swaminathan2015self, kallus2020double}. 
Besides, there is a line of work \citep{liu2018breaking, xie2019towards, kallus2020double, yin2020asymptotically} consider estimating the marginal density ratio of evaluation and target policies, which is called Marginalized Importance Sampling (MIS), and has shown that MIS can help overcome the curse of horizon phenomenon. The third approach DR combines DMM and IS methods by adding estimated value function as error controlling term, which shows a lot of benefits such as lower bias and variance than DM and IS methods \citep{dudik2014doubly, jiang2016doubly, thomas2016data, farajtabar2018more, kallus2020double}. For OFL (or Batch RL), it's more difficult than OPE as the goal of OPL is to learn the optimal policy from the given dataset, especially combining with function approximation settings. When some assumptions are satisfied, many works have discussed the sufficient and necessary conditions of efficient OPL and provided sample efficient algorithms under different function hypothesis classes \citep{munos2008finite, lazaric2012finite, le2019batch,chen2019information, xie2020batch, wang2020statistical, yin2020near, duan2021risk}.

\paragraph{Distributionally Robust Optimization (DRO).} In fact, handling uncertainty set in robust MDPs is relevant with Distributionally Robust Optimization (DRO), where the objective function is minimized with a worst-case loss function. The core motivation of DRO is to deal with the distribution shift of data under different uncertainty sets. \citet{bertsimas2018data, delage2010distributionally} consider the uncertainty set is formulated by moment conditions, while \citet{ben2013robust, duchi2021statistics, duchi2016variance, lam2016robust,duchi2018learning} consider the uncertainty set is formulated by $f$-divergence balls. Besides, \citet{wozabal2012framework, blanchet2019quantifying, gao2016distributionally, lee2017minimax} also consider Wasserstein balls, which is more computationally challenging. The most related work with our results is \citet{duchi2018learning}, where they consider the asymptotic and non-asymptotic performances of the empirical minimizer on a population level. However, the results of \citet{duchi2018learning} are mainly built on the field of supervised learning, while our results are built on robust MDPs. And recently, there is a line of works \citep{jin2020pessimism, dai2020coindice, xiao2021optimality} also considering the connections between pessimistic RL and DRO.
